Stochastic analysis of ocean wave states with and without rogue waves

This work presents an analysis of ocean wave data including rogue waves. A stochastic approach based on the theory of Markov processes is applied. With this analysis we achieve a characterization of the scale dependent complexity of ocean waves by means of a Fokker-Planck equation, providing stochastic information of multi-scale processes. In particular we show evidence of Markov properties for increment processes, which means that a three point closure for the complexity of the wave structures seems to be valid. Furthermore we estimate the parameters of the Fokker-Planck equation by parameter-free data analysis. The resulting Fokker-Planck equations are verified by numerical reconstruction. This work presents a new approach where the coherent structure of rogue waves seems to be integrated into the fundamental statistics of complex wave states.

==> bib.tex <==
\section*{References}
\begin{thebibliography}{50}

\bibitem{Chabchoub2011}
A. Chabchoub , N. P. Hoffmann and N. Akhmediev 2011 {\it PRL} Rogue Wave Observation in a Water Wave Tank,  \textbf{106}, 204502

\bibitem{Solli2007}
 D.R. Solli, C. Ropers, P. Koonath, B. Jalali, Optical rogue waves, Nature 450, 1054-1057 (2007)
 
\bibitem{Akhmediev2010}
N. Akhmediev and E. Pelinovsky, Eur. Phys. J. Special Topics 185, 1-4 (2010)

\bibitem{Moslem2011}
W. M. Moslem, P. K. Shukla, B. Eliasson, Surface plasma rogue waves , 2011 EPL \textbf{96} 25002

\bibitem{BENCHRIET2013}
F.Benchriet, S. A. EL-Tantawy, W. M. Moslem and M. Djebli, Electrostatic rogue waves in a plasma with a relativistic electron beam, J. Plasma Physics (2013), vol. 79, part 5, pp. 847-851.

\bibitem{Veldes2013}
G P Veldes , et al , Electromagnetic rogue waves in beam-plasma interactions,  J. Opt. \textbf{15} (2013) 064003 (10pp)

\bibitem{Dudley2010}
J.M. Dudley , et al, Extreme events in optics: Challenges of the MANUREVA project, Eur. Phys. J. Special Topics  \textbf{185}, 125-133 (2010)

\bibitem{zakharov2010}
V.E. Zakharov , et al, How probability for freak wave formation can be found. Eur. Phys. J. Special Topics \textbf{185}, 113-124 (2010)

\bibitem{Akhmediev2009a}
N. Akhmediev, et al. Waves that appear from nowhere and disappear without a trace. Physics Letters A \textbf{373} (2009) 675-678

\bibitem{Akhmediev2009b}
N. Akhmediev , et al, Matter rogue waves, Phys. Lett. 373, 2137 (2009)

\bibitem{Fedele2007}
F. Fedele, et al, Explaining extreme waves by a theory of stochastic wave groups, Computers and structures 2007 vol,85.pg:291-303

\bibitem{Onorato2002}
M.Onorato,et al, Extreme wave events in directional, random oceanic sea states, Physics of fluids 2002, vol.14, pg:L25-L28

\bibitem{Osborne2001}
A.R. Osborne, et al, Freak waves in random oceanic sea states, Phys. Rev. Lett. 86, 5831-5834 (2001)

\bibitem{Fedele2006}
F.Fedele, et al, Extreme events in nonlinear random seas, Journal of offshore mechanics and Arctic engineering 2006, vol.128, pg:11-16

\bibitem{Onorato2009}
M. Onorato, et al, Statistical Properties of Directional Ocean Waves: The Role of the Modulational Instability in the Formation of Extreme Events, Phys. Rev. Lett. 102, 114502 (2009) [4 pages]

\bibitem{Friedrich1997}
R. Friedrich, et al, Description of a Turbulent Cascade by a Fokker-Planck Equation, Phys.Rev.Lett. \textbf{78}, 863-866 (1997).

\bibitem{Renner2001a}
Ch. Renner, et al, Evidence of Markov properties of high frequency exchange rate data Physica A {\bf 298}, 499 (2001).

\bibitem{Nawroth2010}
A. P. Nawroth , et al, Multi-scale description and prediction of financial time series, New Journal of Physics \textbf{12}, 083021 (2010).

\bibitem{Ghasemi2007}
F. Ghasemi et al, Markov analysis and Kramers-Moyal expansion of nonstationary stochastic processes with application to the fluctuations in the oil pricePhys. Rev. E 75, 060102 ( 2007).

\bibitem{Ghasemi2006}
F. Ghasemi , et al, Analysis of Non-stationary Data for Heart-Rate Fluctuations in Terms of Drift and Diffusion Coefficients. J. Biological Physics 32, 2 (2006) 117-128(12)

\bibitem{Atyabi2006}
F. Atyabi , et al, Two Statistical Methods for Resolving Healthy Individuals and Those with Congestive Heart Failure Based on Extended Self-similarity and a Recursive Method, Biological Physics, 32, 489 (2006)

\bibitem{Soares2003}
Guedes Soares, et al, Characteristics of abnormal waves in north sea storm states. Appl Ocean Res {\bf 25}, 337 (2003)

\bibitem{Haver1998}
Haver S, Karunakaran D. Probabilistic description of crest heights of ocean waves Proceedings of the fifth international workshop on wave hindcasting and forecasting, Melbourne, FL; 1998.

\bibitem{Sand1990}
Sand SE, et al, Freak wave kinematics. In: Torum O, Gudmestad OT, editors. Water wave kinematics. Kluwer Academic Publication; 1990. p. 450-535.

\bibitem{Mori2002a}
N. Mori, et al, Analysis of freak wave measurements in the sea of Japan. Ocean Engineering 29 (2002) 1399-1414.

\bibitem{Divinsky2004}
Divinsky BV, et al, A freak wave in the Black sea: observations and simulation. Dokl Earth Sci 2004;395A:438-43.

\bibitem{Forristall2004}
Forristall GZ, et al, Wave crest sensor intercomparison study: an overview of WACSIS. J. Offshore Mech. Arct. Eng. 126(1), (2004), 26-34 

\bibitem{Mori2002b}
N. Mori, T. Yasuda, Effects of high-order nonlinear wave-wave interactions on gravity waves, Ocean Engineering 29 (2002), 1233-1245.

\bibitem{Mori2002c}
N. Mori, et al,A weakly non-Gaussian model of wave height distribution for random wave train, Ocean Engineering, 29 (2002), 1219-1231.


\bibitem{Liu2000}
P. Liu, N. Mori,  \emph{Characterizing freak waves with wavelet transform analysis} , Rouge Waves 2000, Brest, France, pp.151-156.

\bibitem{Waechter2003}
M. W\"achter, et al. Stochastic analysis of different rough surfaces. Euro Physics Letters pp. 579-585 (2003)

\bibitem{Jafari2003}
G. Jafari , et al. Stochastic analysis and regeneration of rough surfaces. Physical Review Letters 91 (2003).

\bibitem{Tabar2006}
M. Reza Rahimi Tabar , et al. Short-Term Prediction of Medium- and Large-Size Earthquakes Based on Markov and
Extended Self Similarity Analysis of Seismic Data. Lecture Notes in Physics, \textbf{705}, 2006, pp. 281-301

\bibitem{Siegert1998}
S.~Siegert, et al, Analysis of Data of Stochastic Systems, Phys. Lett. A \textbf{243}, 275 (1998)

\bibitem{Friedrich2000}
R.~Friedrich, et al, Extracting model equations from experimental data, Phys. Lett. A \textbf{271}, 217 (2000)
 
\bibitem{Stresing2010} 
R. Stresing, et al, Towards a stochastic multi-point description of turbulence, New Journal of Physics {\bf 12}, 103046 (2010).

\bibitem{Friedrich2011}
R.~Friedrich,et al, Approaching Complexity by Stochastic Methods: From Biological Systems to Turbulence, Physics Reports \textbf{506},
 87 (2011)
 
\bibitem{Einstein1905} A. Einstein, 
{\em \"Uber die von der molekularkinetischen Theorie der W\"arme
geforderte Bewegung von in ruhenden Fl\"ussigkeiten suspendierten
Teilchen} Ann. Phys. {\bf 17}, 549 (1905).
 
 \bibitem{Kolmogorov1931}
 A.N. Kolmogorov, \"Uber die analytischen Methoden in der Wahrscheinlichkeitsrechnung, Mathematische Annalen 104 (1931) \textbf{415},
 
 \bibitem{Risken1989}
H. Risken, The Fokker$-$Planck Equation , 2nd ed., Springer, Berlin, 1989.

\bibitem{huang1998a}
N. E. Huang, et al, The empirical mode decomposition and the Hilbert spectrum for nonlinear and non-stationary time series analysis. Proc. R. Soc. Land. A (1998) 454, 903-995

\bibitem{huang1998b}
W. Huang, et al , Engineering Analysis of Intrinsic Mode and Indicial Response in Biology: the Transient Response of Pulmonary Blood Pressure to Step Hypoxia and Step Recovery, Proc of the National Academy of Science,USA,95(1998) 12766-12771.

\bibitem{huang1999a}
N. E. Huang, et al, A NEW VIEW OF NONLINEAR WATER WAVES: The Hilbert Spectrum, Annu. Rev. Fluid Mech. 1999. 31:417-57 .

\bibitem{huang2007}
N. E. Huang, et al, Application of the empirical mode decomposition and Hilbert - Huang transform to seismic reflection data, GEOPHYSICS, VOL. 72. NO. 2 (2007); P. H29-H37, 12 FIGS.

\bibitem{Nunes2003}
J. Nunes, et al, Image analysis by bidimensional em- pirical mode decomposition, Image and Vision Computing, 21(12)(2003) 1019-1026.



\bibitem{huang2003}
N. E. Huang, et al, Applications of Hilbert-Huang transform to non-stationary financial time series analysis. APPLIED STOCHASTIC MODELS IN BUSINESS AND INDUSTRY, Appl. Stochastic Models Bus. Ind.2003; 19:245-268 (DOI: 10.1002/asmb.501)

\bibitem{huang1998c}
N. E. Huang, et al, The empirical mode decomposition and the Hilbert Spectrum for nonlinear and non-stationary time series analysis. Proceedings of the Royal Society
London 1998; A454:903-995.


\bibitem{huang1999b}
N. E. Huang, et al, Computer Implemented Empirical Mode Decomposition Method, Apparatus, and Article of Manufacture. (US Provisional Application Serial 
Number 60/023,411, August 14, 1966 and Serial No. 60/023,822 filed on August 12,1996, US Patent 5,983, 162 November, 1999.)

\bibitem{Renner2001b} C. Renner, et al, Experimental indications for Markov properties of small-scale turbulence, J. Fluid Mech. {\bf 433}, 383 (2001).

\bibitem{Nick2013} D. Nickelsen et al, Probing Small-Scale Intermittency with a Fluctuation Theorem, Phys. Rev. Lett. {\bf 110}, 214501 (2013)

\end{thebibliography}

\end{document}


